Alternating Linearization for Structured Regularization Problems

We adapt the alternating linearization method for proximal decomposition to structured regularization problems, in particular, to the generalized lasso problems. The method is related to two well-known operator splitting methods, the Douglas--Rachford and the Peaceman--Rachford method, but it has descent properties with respect to the objective function. This is achieved by employing a special update test, which decides whether it is beneficial to make a Peaceman--Rachford step, any of the two possible Douglas--Rachford steps, or none. The convergence mechanism of the method is related to that of bundle methods of nonsmooth optimization. We also discuss implementation for very large problems, with the use of specialized algorithms and sparse data structures. Finally, we present numerical results for several synthetic and real-world examples, including a three-dimensional fused lasso problem, which illustrate the scalability, efficacy, and accuracy of the method.

==> AL-AR.bib.tex <==
@article{Li09,
  author = "C. Li, W. Yin, H. Jiang, and Y. Zhang",
  title = "An Ecient Augmented Lagrangian Method
with Applications to Total Variation Minimization",
  journal = "Computational Optimization and Applications",
  year="2013",
  volume = 56,
  number=03
}
@article{Wright09,
  author = "S. Wright and R. Nowak and M. Figueiredo",
  title = "Sparse Reconstruction by Separable Approximation",
  journal = "IEEE TRANSACTIONS ON SIGNAL PROCESSING",
  year="2009",
  volume = 57,
  number=07
}
@article{Wahlberg12,
  author = "B. Wahlberg, S. Boyd, M. Annergren, Y. Wang",
  title = "An ADMM Algorithm for a Class of Total Variation Regularized Estimation Problems",
  journal = "arXiv:1203.1828",
  year="2012",
}
@article{Zhang12,
  author = "Z. Zhang and K. Lange and C. Sabatti",
  title = "Reconstructing DNA copy number by joint segmentation of multiple sequences",
  journal = "BMC Bioinformatics",
  year="2012",
  volume = 13,
  number=205
}
@article{Michel11,
  author = "V. Michel and A. Gramfort and G. Varoquaux and E. Eger and B. Thirion",
  title = "Total Variation Regularization for fMRI-Based Prediction of Behavior",
  journal = "IEEE Transactions on Medical Imaging",
  year="2011",
  volume = 30,
  number=7,
  pages="1328-1340"
}

@article{Wang08,
  author = "Y. Wang and J. Yang and W. Yin and Y. Zhang",
  title = "A New Alternating Minimization Algorithm for Total Variation Image Reconstruction",
  journal = "SIAM Journal on Imaging Sciences",
  year="2008",
  volume = 1,
  number=3,
  pages="248-272"
}

@article{Grosenick11,
  author = "L. Grosenick and B. Klingenberg and B. Knutson and J. Taylor",
  title = "A family of interpretable multivariate models for regression and classification of whole-brain fMRI data",
  year="2011",
eprint="arXiv/1110.4139",
doi=""
}

@article{Beck09,
  author = "A. Beck and M. Teboulle",
  title = "A fast iterative shrinkage-thresholding algorithm for linear inverse problems",
  journal = "SIAM Journal on Imaging Sciences",
  year="2009",
  volume = 2,
  number=1,
  pages = "183-202"
}

@book{Bertsekas95,
  author = "D. Bertsekas",
  title = "Nonlinear programming",
  journal = "Athena Scientific",
  year = "1995"
}

@article{Tib96,
  author = "R. Tibshirani",
  title = "Regression shrinkage and selection via the lasso",
  journal = "Journal of The Royal Statistical Society Series B",
  volume = 58,
  number=1,
  pages = "267-288",
  year = "1996"
}

@article{Fu98,
  author = "W. Fu",
  title = " Penalized regressions: the bridge vs. the Lasso",
  journal = " Journal of Computational and Graphical Statistics",
  volume = 7,
  number = 3,
  pages = "397-416",
  year = "1998"
}

@article{Friedman07,
  author = "J. Friedman and T. Hastie and H. Hoefling and R. Tibshirani",
  title = "Pathwise coordinate optimization",
  journal = "Annals of Applied Statistics",
  volume = 1,
  number = 2,
  pages = "302-332",
  year = "2007"
}

@article{Daub04,
  author = "I. Daubechies and M. Defrise and C. De Mol",
  title = " An iterative thresholding algorithm for linear inverse problems with a sparsity constraint",
  journal = "Comm. Pure Appl. Math",
  volume = 57,
  number = 11,
  pages = "1413-1457",
  year = "2004"
}

@article{Efron04,
  author = "B. Efron and T. Hastie and I. Johnstone and R. Tibshirani",
  title = {Least angle regression},
  journal = "Annals of Statistics",
  volume = 32,
  number = 2,
  pages = "407-451",
  year = "2004"
}

@article{Yuan06,
  author = "M. Yuan and Y. Lin",
  title = "Model selection and estimation in regression with grouped variables",
  journal = "Journal of The Royal Statistical Society Series B",
  volume = 68,
  number = 1,
  pages = "49-67",
  year = "2006"
}

@article{Tib05,
  author = "R. Tibshirani and M. Saunders and J. Zhu and S. Rosset",
  title = "Sparsity and smoothness via the fused lasso",
  journal = "Journal of The Royal Statistical Society Series B",
  volume = 67,
  pages = "91-108",
  year = "2005"
}

@article{Tib11,
  author = "R. Tibshirani and J. Taylor",
  title = "The Solution Path of the Generalized Lasso",
  journal = "Annals of Statistics",
  year = "2011"
}

@article{Jun10,
  author = "J. Liu and L. Yuan and J. Ye",
  title = "An Efficient Algorithm for a Class of  Fused Lasso Problems",
  journal = "ACM SIGKDD Conference on Knowledge Discovery and Data Mining",
  year="2010"
}

@techreport{Jun11,
  author = "J. Liu and L. Yuan and J. Ye",
  title = "{SLEP}: Sparse Learning with Efficient Projections",
  type = "techincal report",
  institution = "Computer Science Center, Arizona State University",
  year="2011"
}

@techreport{Nesterov,
  author = "Nesterov, Yu.",
  title = "Gradient methods for minimizing composite objective function",
  type = "discussion paper 2007/76",
  institution = "CORE",
  year="2007"
}

@article{Hoefling10,
  author = "H. Hoefling",
  title = "A path algorithm for the Fused Lasso Signal Approximator",
  journal = "Journal of Computational and Graphical Statistics",
  volume = 19,
  number = 4,
  page ="984-1006",
  year = "2010"
}

@article{Tseng01,
  author = "P. Tseng",
  title = "Convergence of block coordinate descent method for nondifferentiable minimization",
  journal = "Journal of Optimization Theory and Applications",
  volume = 109,
  pages = "474-494",
  year = "2001"
}


@article{Kiwiel99,
  author = "K. Kiwiel and C. Rosa and A. Ruszczy\'nski",
  title = "Proximal decomposition via alternating linearization",
  journal = "SIAM Journal on Optimization",
  volume = 9,
  pages = "153-172",
  year = "1999"
}
@article{Prasa10,
author="P. Karunanayaka and V. J. Schmithorst and J. Vannest and J. P. Szaflarski and E. Plante and S. K.  Holland",
title = "A group independent component analysis of covert verb generation in children: A functional magnetic resonance imaging study",
journal="Neuroimage",
year="2010",
volume= "51",
pages = "472-487"
}

@article{Schmithorst06,
author="V. Schmithorst and S. Holland and E. Plante",
title="Cognitive modules utilized for narrative comprehension in children: a functional magnetic resonance imaging study",
journal="Neuroimage",
volume=29,
pages="254-266",
year="2006"
}

@article{Kim10,
  author = "S. Kim and E. Xing",
  title = "Tree-Guided Group Lasso for Multi-Task Regression with Structured Sparsity",
  journal = "The 27th International Conference on Machine Learning",
  year = "2010"
}

@techreport{Chen11,
author="X. Chen and S. Kim and Q. Lin and J. Carbonell and E. Xing",
 title = "An Efficient Proximal Gradient Method for General Structured Sparse Learning",
type = "technical report 1005.4717v3",
institution="arXiv",
year="2011"
}
@techreport{Chen10,
author="X. Chen and S. Kim and Q. Lin and J. Carbonell and E. Xing",
title="Graph-Structured Multi-task Regression and an Efficient Optimization Method for General Fused Lasso",
type = "technical report 1005.3579v1",
institution="arXiv",
year="2010"
}

@techreport{Argyriou,
author="A. Argyriou and C. A. Micchelli and M. Pontil and L. Shen and Y. Xu",
title="Efficient First Order Methods for Linear Composite Regularizers",
type = "technical report 1104.1436v1",
institution="arXiv",
year="2011"
}


@techreport{Combettes-Pesquet,
author="P. L. Combettes and J.-C. Pesquet",
type = "technical report 0912.3522v4",
title="Proximal Splitting Methods in Signal Processing",
institution="arXiv",
year="2010"
}

@article {Combettes2009,
    AUTHOR = {Combettes, P. L.},
     TITLE = {Iterative construction of the resolvent of a sum of maximal
              monotone operators},
   JOURNAL = {J. Convex Anal.},
  FJOURNAL = {Journal of Convex Analysis},
    VOLUME = {16},
      YEAR = {2009},
    NUMBER = {3-4},
     PAGES = {727--748},
}

@book{Bauschke-Combettes,
    AUTHOR = {Bauschke, H. H. and Combettes, P. L.},
     TITLE = {Convex analysis and monotone operator theory in {H}ilbert
              spaces},
    SERIES = {CMS Books in Mathematics/Ouvrages de Math\'ematiques de la
              SMC},
 PUBLISHER = {Springer},
   ADDRESS = {New York},
      YEAR = {2011},
}
@article {Lions-Mercier,
    AUTHOR = {Lions, P.-L. and Mercier, B.},
     TITLE = {Splitting algorithms for the sum of two nonlinear operators},
   JOURNAL = {SIAM J. Numer. Anal.},
  FJOURNAL = {SIAM Journal on Numerical Analysis},
    VOLUME = {16},
      YEAR = {1979},
    NUMBER = {6},
     PAGES = {964--979},
}
@article {Eckstein-Bertsekas,
    AUTHOR = {Eckstein, J. and Bertsekas, D. P.},
     TITLE = {On the {D}ouglas-{R}achford splitting method and the proximal
              point algorithm for maximal monotone operators},
   JOURNAL = {Math. Programming},
  FJOURNAL = {Mathematical Programming},
    VOLUME = {55},
      YEAR = {1992},
    NUMBER = {3, Ser. A},
     PAGES = {293--318},
}
@article {Peaceman-Rachford,
    AUTHOR = {Peaceman, D. W. and Rachford,  H. H.},
     TITLE = {The numerical solution of parabolic and elliptic differential
              equations},
   JOURNAL = {J. Soc. Indust. Appl. Math.},
    VOLUME = {3},
      YEAR = {1955},
     PAGES = {28--41},
}
@article {Douglas-Rachford,
    AUTHOR = {Douglas, J. and Rachford,  H. H.},
     TITLE = {On the numerical solution of heat conduction problems in two
              and three space variables},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {82},
      YEAR = {1956},
     PAGES = {421--439},
}

@article {Ruszczynski95,
    AUTHOR = {Ruszczy{\'n}ski, A.},
     TITLE = {On convergence of an augmented {L}agrangian decomposition
              method for sparse convex optimization},
   JOURNAL = {Math. Oper. Res.},
  FJOURNAL = {Mathematics of Operations Research},
    VOLUME = {20},
      YEAR = {1995},
    NUMBER = {3},
     PAGES = {634--656},
}
@article {Ye-Xie,
    AUTHOR = {Ye, G.-B. and Xie, X.},
     TITLE = {Split {B}regman method for large scale fused {L}asso},
   JOURNAL = {Comput. Statist. Data Anal.},
  FJOURNAL = {Computational Statistics \& Data Analysis},
    VOLUME = {55},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {1552--1569},
}
@article {Goldstein-Osher,
    AUTHOR = {Goldstein, T. and Osher, S.},
     TITLE = {The split {B}regman method for {$L1$}-regularized problems},
   JOURNAL = {SIAM J. Imaging Sci.},
  FJOURNAL = {SIAM Journal on Imaging Sciences},
    VOLUME = {2},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {323--343},
}
@article{Boyd-et-al,
    AUTHOR = { Boyd, S. and Parikh,  N. and  Chu, E. and Peleato, B. and Eckstein, J. },
     TITLE = {Distributed Optimization and Statistical Learning via the Alternating Direction Method of Multipliers},
   JOURNAL = {Foundations and Trends in Machine Learning},
    VOLUME = {3},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {1--122},
}
@book {Golub-VanLoan,
    AUTHOR = {Golub, G. H. and Van Loan, C. F.},
     TITLE = {Matrix Computations},
    SERIES = {Johns Hopkins Studies in the Mathematical Sciences},
   EDITION = {Third},
 PUBLISHER = {Johns Hopkins University Press},
   ADDRESS = {Baltimore, MD},
      YEAR = {1996},
}
@article {Birgin-Martinez,
    AUTHOR = {Birgin, E. G. and Mart{\'{\i}}nez, J. M.},
     TITLE = {Large-scale active-set box-constrained optimization method
              with spectral projected gradients},
   JOURNAL = {Comput. Optim. Appl.},
  FJOURNAL = {Computational Optimization and Applications. An International
              Journal},
    VOLUME = {23},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {101--125},
}
@ARTICLE{Fadili-Peyre,
 author={Fadili, J.M. and Peyr\'{e}, G.},
 journal={IEEE Transactions on Image Processing},
 title={Total Variation Projection With First Order Schemes},
 year={2011},
 volume={20},
 number={3},
 pages={657 -669},
 }
 @book {Rusz-book,
    AUTHOR = {Ruszczy{\'n}ski, A.},
     TITLE = {Nonlinear optimization},
 PUBLISHER = {Princeton University Press},
   ADDRESS = {Princeton, NJ},
      YEAR = {2006},
}
@book {BGLS-book,
    AUTHOR = {Bonnans, J. F. and Gilbert, J. C. and
              Lemar{\'e}chal, C. and Sagastiz{\'a}bal, C. A.},
     TITLE = {Numerical optimization, Theoretical and practical aspects},
    SERIES = {Universitext},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
}
@book {Kiwiel-book,
    AUTHOR = {Kiwiel, K. C.},
     TITLE = {Methods of descent for nondifferentiable optimization},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1133},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1985},
}

@article{Tibshirani-Wang,
author = {Tibshirani, R. and Wang, P.},
title = {Spatial smoothing and hot spot detection for CGH data using the fused lasso},
volume = {9},
number = {1},
pages = {18-29},
year = {2008},
journal = {Biostatistics}
}
@article{Friedlander-Martinez,
    AUTHOR = {Friedlander, A. and Mart{\'{\i}}nez, J. M.},
     TITLE = {On the maximization of a concave quadratic function with box
              constraints},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {4},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {177--192},
}
@incollection {Birgin-Martinez-2001,
    AUTHOR = {Birgin, E. G. and Mart{\'{\i}}nez, J. M.},
     TITLE = {A box-constrained optimization algorithm with negative
              curvature directions and spectral projected gradients},
 BOOKTITLE = {Topics in numerical analysis},
    SERIES = {Comput. Suppl.},
    VOLUME = {15},
     PAGES = {49--60},
 PUBLISHER = {Springer},
   ADDRESS = {Vienna},
      YEAR = {2001},
}
@article {Birgin-Martinez-Raydan,
    AUTHOR = {Birgin, E. G. and Mart{\'{\i}}nez, J. M. and
              Raydan, M.},
     TITLE = {Nonmonotone spectral projected gradient methods on convex
              sets},
   JOURNAL = {SIAM J. Optim.},
  FJOURNAL = {SIAM Journal on Optimization},
    VOLUME = {10},
      YEAR = {2000},
    NUMBER = {4},
     PAGES = {1196--1211},
}
@article{Friedlander-Martinez-Raydan,
    AUTHOR = {Friedlander, A. and  Mart{\'{\i}}nez, J. M., and M. Raydan},
     TITLE = {SPG: Software for convex-constrained optimization},
   JOURNAL = {ACM Transactions on Mathematical Software},
    VOLUME = {27},
      YEAR = {2001},
     PAGES = {340--349},
}
@book {HUL-book,
    AUTHOR = {Hiriart-Urruty, J.-B. and Lemar{\'e}chal, C.},
     TITLE = {Convex analysis and minimization algorithms. {II}},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {306},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {1993},
}

@techreport{He-Yuan,
  author = "B. He and X. Yuan",
  title = "On the {$O(1/t)$} convergence rate of alternating direction method",
  type = "technical report",
  institution = "Optimization On-Line",
  year="2011"
}

